Kindly Bent to Free Us

Systems programming often requires the manipulation of resources like file handles, network connections, or dynamically allocated memory. Programmers need to follow certain protocols to handle these resources correctly. Violating these protocols causes bugs ranging from type mismatches over data races to use-after-free errors and memory leaks. These bugs often lead to security vulnerabilities. While statically typed programming languages guarantee type soundness and memory safety by design, most of them do not address issues arising from improper handling of resources. An important step towards handling resources is the adoption of linear and affine types that enforce single-threaded resource usage. However, the few languages supporting such types require heavy type annotations. We present Affe, an extension of ML that manages linearity and affinity properties using kinds and constrained types. In addition Affe supports the exclusive and shared borrowing of affine resources, inspired by features of Rust. Moreover, Affe retains the defining features of the ML family: it is an impure, strict, functional expression language with complete principal type inference and type abstraction. Affe does not require any linearity annotations in expressions and supports common functional programming idioms.

==> fig-for-loop-implementation.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.5\linewidth}
\begin{lstlisting}
let for f a  = 
  let n = Array.length &a in
  let rec loop f a i = 
    if i < n then (
      f &!a i;
      loop f &!a (i+1)
    )
  in
  loop f &!a 0
# for : Borrowed m ('a Array.t) tt =>
  (tt -> int -> unit) -> tt -> unit
\end{lstlisting}
    \caption{For loop function for affine arrays}
    \label{ex:array:for}
  \end{subfigure}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-reduction.tex <==
\begin{figure*}[tp]
  % \input{semantics}
    \begin{mathpar}
      \ruleTimeOut

    \ruleSConst

    \ruleSVar

    \ruleSTApp

    \ruleSPLam
    
    \ruleSApp
    
    \ruleSLet

    \ruleSPair
  \end{mathpar}
  \caption{Reduction rules -- lambda calculus fragment
    -- $\Store, \Perm, \VEnv \vdash e \Downarrow  \Store', \Perm', r$
  }
  \label{fig:reduction}
\end{figure*}
\begin{figure*}
  \begin{mathpar}
    \ruleSMatchLocation

    \ruleSMatchBorrow

    \ruleSRegion

    \ruleSBorrow
    \\
    \ruleSCreate

    \ruleSDestroy

    \ruleSObserve

    \ruleSUpdate
  \end{mathpar}
  \caption{Reduction rules -- resource handling
    -- $\Store, \Perm, \VEnv \vdash e \Downarrow  \Store', \Perm', r$
  }
  \label{fig:reduction-resources}
\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> infer/validity.tex <==
\begin{mathpar}
  \inferrule[TyVar]
  { \bvar{\alpha}{k}\in\E }
  { \tyval{C}{\E}{\alpha} }
  \and
  \inferrule[TyArrow]
  { \tyval{C}{\E}{\tau_0} \\
    \tyval{C}{\E}{\tau_1}
  }
  { \tyval{C}{\E}{\tau_0\tarr{k}\tau_1} }
  \and
  \inferrule[TyApp]
  { \bvar{t}{\forall\kvar_j^*.(\qual{D}{k^* \karr k})}\in\E \\
    \entail{C}{\subst{\kvar_j}{k_i}{D}} \\
    \forall i, \tyval{C}{\E}{\tau_i}
  }
  { \tyval{C}{\E}{\tapp{\tcon}{k_i^* \tau_i^*}} }
  \\
  \inferrule[TyScheme]
  { \tyval{C \Cand D}
    {\E;\bkind{\kvar_i}^*;\bvar{\alpha_j}{k_j}^*}{\tau} }
  { \schval{C}{\E}{\forall\kvar_i^*\forall\bvar{\alpha_j}{k_j}^*.(\qual{D}{\tau})} }
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> leftover-metatheory.tex <==
\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  The proof is by induction on the evaluation judgment $\Store, \Perm,
  \VEnv \vdash {e} \Downarrow^i R$.
  
  The base case is trivial as $\Store, \Perm, \VEnv \vdash {e}
  \Downarrow^0 \TimeOut$.

  For indexes greater than zero we have a case distinction over all applicable execution
  rules.

  \textbf{Case }$\ruleSConst$.
  The claim is immediate.

  \textbf{Case }$\ruleSVar$.
  The claim is immediate.

  \textbf{Case }$\ruleSTApp$.
  
  By assumption, we have that $\SE \vdash \Loc : \E (x)$ so that
  $\E(x) =
  \forall\Multi\kvar\forall\Multi{\bvar{\alpha}{k}}.(\qual{C}{\tau_2\tarr{k}\tau_1})$.
  All conclusions hold: $\SE \le \SE' = \SE[\Loc' \mapsto
  (\tau_2\tarr{k}\tau_1)[\Multi[i]{\kvar} \mapsto \Multi[i]{ k},
  \Multi[j]{\alpha} \mapsto \Multi[j]{t}]]$;
  $\vdash \Store' : \SE'$;
  $\Perm' \subseteq \Dom{\Store'}$;
  $\SE' \vdash \Loc' : \tau$;
  and $\Loc' \in \Perm' \Sadd{\Loc'}$.

  \textbf{Case }$\ruleSPLam$.

  By assumption $\SE \vdash     \ilam {\Multi[i]{\kvar}}{\Multi[j]{\tvar}}Ck xe
  : \schm$ where $\schm =
  \forall\Multi\kvar\forall\Multi{\bvar{\alpha}{k}}.(\qual{C}{\tau_2\tarr{k}\tau_1})$. Let
  $\SE'  = \SE[\Loc \mapsto \schm]$.
  Then $\SE \le \SE'$ and $\vdash\Store' : \SE'$.
  Moreover, $\SE' \vdash \Loc : \schm$ and $\Loc \in \Perm
  \Sadd{\Loc}$ as required.
  
  \clearpage
  \textbf{Case }$\ruleSApp$.

  By assumption $\ruleSDApp$.

  \begin{itemize}
  \item By splitting of $\E$, we have that $\VEnv = \VEnv_1 +
    \VEnv_1'$ such that  $\SE \vdash \VEnv_1 : \E_1$
  \item $\vdash \Store : \SE$
  \item $\Reach\Store{\VEnv_1} \subseteq \Reach\Store{\VEnv} \subseteq
    \Perm \subseteq \Dom\Store$ 
  \item $\Rawloc{\VEnv_1'} \subseteq \Dom\Store$ and
    $\Dom{\VEnv_1} \cap \Dom{\VEnv_1'}=\emptyset$
  \item $\Store, \Perm, \VEnv_1 + \VEnv_1' \vdash {e_1}
    \Downarrow^i R_1$
  \end{itemize}
  If $R_1 = \TimeOut$, then $R = \TimeOut$, too.
  Otherwise induction yields that
  $\exists$ $\Store_1$, $\Perm_1$, $r_1$, $\SE_1$ such that
  \begin{itemize}
  \item
    $R_1 = \Ok{\Store_1, \Perm_1, r_1}$  
  \item $\SE \le \SE_1$, $\Store \le \Store_1$,
    $\vdash \Store_1 : \SE_1$ 
  \item $\Perm_1 \subseteq \Dom{\Store_1}$
  \item $\SE_1 \vdash r_1 : \tau_2\tarr{k}\tau_1$
  \item $\Reach{\Store_1}{r_1} \subseteq \Perm_1$ and by inverting the
    previous typing, we 
    know that $r_1 = \Loc$ hence $\Loc \in \Perm_1$ 
  \item For all $\Loc \in \Reach{\Store_1}{\VEnv_1'}$ it
    must be that $\Store_1 (\Loc) = \Store (\Loc)$ and
    $\Loc\in\Perm \Leftrightarrow \Loc\in\Perm_1$
  \end{itemize}
  By inversion of the store typing we also know that $\Store_1 (\Loc)
  = (\VEnv'',\lam[k]{x}{e})$, for some $\VEnv''$, $k$, $x$, and
  $e$.
  To establish the assumptions for the evaluation for $e_2$, we reason
  as follows
  \begin{itemize}
  \item By splitting of $\E$, we have that $\VEnv = \VEnv_2 +
    \VEnv_2'$ such that  $\SE_1 \vdash \VEnv_2 : \E_2$ (because $\SE\le\SE_1$)
  \item $\vdash \Store_1 : \SE_1$ (by the previous IH)
  \item $\Perm_1' \subseteq \Dom{\Store_1}$ (by the previous IH)
  \item To see that
    $\Reach{\Store_1}{\VEnv_2} \subseteq \Perm_1'$ \\
    Suppose that $\Loc' \in \Reach{\Store_1}{\VEnv_2}$.
    \begin{itemize}
    \item If $\Loc' \in \Reach{\Store_1}{\VEnv_1'} \subseteq
      \Reach\Store{\VEnv_1'} \subseteq \Reach\Store\VEnv$, then $\Loc'
      \in \Perm_1'$ (as $\Loc' \ne \Loc$ which is either new or taken
      from $\Reach{\Store_1}{\VEnv_1}$).
    \item If
      $\Loc \in \Reach{\Store_1}{\VEnv_1'} \cap
      \Reach{\Store_1}{\VEnv_1}$, then ${\entail {} {k \le \kun}}$
      must hold by splitting, which means that $\Loc$ is not writeable
      so that $\Loc\in\Perm_1'$.
    \item If $\Loc' \in \Reach{\Store_1}{\VEnv_1}$, then splitting
      enforces that $\neg\Writeable{\SE_1}{\Loc'}$, hence $\Loc' \in \Perm_1'$.
    \end{itemize}
  \item $\Rawloc{\VEnv_2'} \subseteq \Dom{\Store} \subseteq \Dom{\Store_1}$ and
    $\Dom{\VEnv_2} \cap \Dom{\VEnv_2'}=\emptyset$ by construction
  \item $\Store_1, \Perm_1', \VEnv_2 + \VEnv_2' \vdash {e_2}
    \Downarrow^i R_2$
  \end{itemize}
  If $R_2 = \TimeOut$, then $R = \TimeOut$, too.
  Otherwise induction yields that
  $\exists$ $\Store_2$, $\Perm_2$, $r_2$, $\SE_2$ such that
  \begin{itemize}
  \item
    $R_2 = \Ok{\Store_2, \Perm_2, r_2}$  
  \item $\SE_1 \le \SE_2$, $\Store_1 \le \Store_2$,
    $\vdash \Store_2 : \SE_2$ 
  \item $\Perm_2 \subseteq \Dom{\Store_2}$
  \item $\SE_2 \vdash r_2 : \tau_2$
  \item $\Reach{\Store_2}{r_2} \subseteq \Perm_2$
  \item For all $\Loc \in \Reach{\Store_2}{\VEnv_2'}$ it must be that
    $\Store_2 (\Loc) = \Store_1 (\Loc)$
    and $\Loc\in\Perm_1' \Leftrightarrow \Loc\in\Perm_2$ 
  \item For all $\Loc \in \Reach{\Store_2}{\VEnv_2}$,
    if $\neg \Writeable{\SE_2}\Loc $ then
    $\Store_2 (\Loc) = \Store_1 (\Loc)$
    and $\Loc\in\Perm_1' \Leftrightarrow \Loc\in\Perm_2$ 
  \end{itemize}

  It remains to establish the assumptions for the evaluation of $e$.
  \begin{itemize}
  \item $\exists C'', \E''$ such that
    $\inferS{C''}{\E'';\bvar{x}{\tau_2}}{e}{\tau_1}$ and
    $\addlin{\entail{C''}{\Cleq{\E''}{k}}}$
  \item Moreover $\SE_2 \vdash \VEnv'' : \E''$ because $\SE \le \SE_2$
  \item $\vdash \Store_2 : \SE_2$ \quad (by previous IH)
  \item $\Perm_2 \subseteq \Dom{\Store_2}$
  \item To see that $\Reach{\Store_2}{\VEnv''}\subseteq \Perm_2$:
  \\
  Suppose that $\Loc' \in \Reach{\Store_2}{\VEnv''}$.
  Clearly $\Loc' \in \Reach{\Store_1}{\Loc}$, the address of the
  closure, and $\Loc' \in \Perm_1'$ by the inductive hypothesis for
  evaluating $e_1$.
  \begin{itemize}
  \item If $\neg\Writeable{\SE_2}{\Loc'}$,
    then $\Loc' \in \Perm_2$ (because it was never removed from
    $\Perm$)
  \item If $\Writeable{\SE_2}{\Loc'}$, then $k$ must be restricted and
    evaluation of $e_2$ could not remove it from $\Perm_2$ because
    $\Loc' \notin \Reach{\Store_1}{\VEnv_1}$.
  \end{itemize}
  \item For $\VEnv'$ we take $\emptyset$, which fulfills all assumptions
  \item $\Store_2, \Perm_2, \VEnv'' + \emptyset \vdash {e}\Downarrow^i R_3$
  \end{itemize}
  If $R_3 = \TimeOut$, then $R = \TimeOut$, too.
  Otherwise induction yields that
  $\exists$ $\Store_3$, $\Perm_3$, $r_3$, $\SE_3$ such that
  \begin{itemize}
  \item
    $R_3 = \Ok{\Store_3, \Perm_3, r_3}$  
  \item $\SE_2 \le \SE_3$, $\Store_2 \le \Store_3$,
    $\vdash \Store_3 : \SE_3$ 
  \item $\Perm_3 \subseteq \Dom{\Store_3}$
  \item $\SE_3 \vdash r_3 : \tau_1$
  \item $\Reach{\Store_3}{r_3} \subseteq \Perm_3$
  \item Frame condition is void as the ignored part of the environment
    is $\emptyset$.
  \end{itemize}

  From the above, we need to conclude that
  $\exists$ $\Store' = \Store_3$, $\Perm' = \Perm_3$, $r' = r_3$,
  $\SE' = \SE_3$ such that
  \begin{itemize}
  \item
    $R = \Ok{\Store', \Perm', r'}$  
  \item $\SE \le \SE'$, $\Store \le \Store'$,
    $\vdash \Store' : \SE'$, the first two by transitivity of $\le$
    and the last by the IH for evaluating $e$
  \item $\Perm' \subseteq \Dom{\Store'}$ (by last IH)
  \item $\SE' \vdash r' : \tau_1$ (by last IH)
  \item $\Reach{\Store'}{r'} \subseteq \Perm'$ (by last IH)
  \item For all $\Loc \in \Reach{\Store'}{\VEnv'}$ it must be that
    $\Store' (\Loc) = \Store (\Loc)$
    and $\Loc\in\Perm \Leftrightarrow \Loc\in\Perm'$ 
  \item For all $\Loc \in \Reach{\Store'}{\VEnv}$,
    if $\neg \Writeable{\SE'}\Loc $ then
    $\Store' (\Loc) = \Store (\Loc)$
    and $\Loc\in\Perm \Leftrightarrow \Loc\in\Perm'$ 
  \end{itemize}
  

  \clearpage
  \textbf{Case }$\ruleSLet$.

  \textbf{Case }$\ruleSPair$.

  \textbf{Case }$\ruleSMatchLocation$.

  \textbf{Case }$\ruleSMatchBorrow$.

  \clearpage
  \textbf{Case }$\ruleSRegion$.

  We assume that
  \begin{itemize}
  \item $\inferS{C}{\E}{\region{\Sone x \BORROW}{e}}{\tau}$
  \item $\SE \vdash \VEnv, \MutableBorrows\VEnv : \E$ \\
    ($\MutableBorrows\VEnv$ contains suspended
    bindings which we cannot use, although we have the permission)
  \item $\vdash \Store : \SE$
  \item $\Reach\Store{\VEnv, \MutableBorrows\VEnv} \subseteq \Perm \subseteq \Dom\Store$\\
    (we have permission for suspended bindings)
  \item  $\VEnv'$ with $\Rawloc{\VEnv'}
    \subseteq \Dom\Store$ and $\Dom\VEnv \cap \Dom{\VEnv'}=\emptyset$
    \\
    (that would be the enclosing frame)
  \item  $i\in\Nat$ and $\Store, \Perm, \VEnv + \MutableBorrows\VEnv +
    \VEnv' \vdash {\region{\Sone x \BORROW}{e}}
    \Downarrow^{i+1} R$ and $R\ne \TimeOut$.
  \end{itemize}
  
  We apply inversion to the typing: 
  
  $\ruleSDRegion$.

  We see that $x \in \Dom{\MutableBorrows\VEnv}$.
  
  Hence, $\E'$ is mostly equal to $\E$ but $\svar x{\tau_x}$ is
  replaced by $\bvar {\borrow x}{\borrowty{k} {\tau_x}}$.

  (PT: but how is $k$ chosen? Is it $k_\tau$?)

  So $\VEnv' = \VEnv[x \mapsto \MutableBorrows\VEnv (x)b]$ and
  $\MutableBorrows\VEnv' = \MutableBorrows\VEnv \Sdel x$

\clearpage
  \textbf{Case }$\ruleSBorrow$.

  \textbf{Case }$\ruleSCreate$.

  \textbf{Case }$\ruleSDestroy$.

  \textbf{Case }$\ruleSObserve$.

  \textbf{Case }$\ruleSUpdate$.
\end{proof}


==> lst-rule.tex <==
% Don't ask me
% https://tex.stackexchange.com/questions/445691/spacing-issue-with-literate-in-listings
\makeatletter
\def\lst@Literate#1#2#3{%
    \ifx\relax#2\@empty\else
        \lst@CArgX #1\relax\lst@CDef
            {}
            {\let\lst@next\@empty
             \lst@ifxliterate
                \lst@ifmode \let\lst@next\lst@CArgEmpty \fi
             \fi
             \ifx\lst@next\@empty
                 \ifx\lst@OutputBox\@gobble\else
                   \lst@XPrintToken \let\lst@scanmode\lst@scan@m
                   \lst@token{#2}\lst@length#3\relax
                   \lst@XPrintToken
                   \lst@whitespacefalse %!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
                 \fi
                 \let\lst@next\lst@CArgEmptyGobble
             \fi
             \lst@next}%
            \@empty
        \expandafter\lst@Literate
    \fi}
\makeatother

\lstdefinestyle{rule}{
  language=Caml,
  showstringspaces=false,
  basicstyle=\small\normalfont,
  keywordstyle=\textbf,
  columns=[c]fullflexible,
  flexiblecolumns,
  % If you want to keep a monospace code-like style:
  % basicstyle=\ttfamily,
  % columns=[c]spaceflexible,
  % flexiblecolumns=false,
  aboveskip=0pt,
  belowskip=0pt,
  lineskip=-1pt,
  showlines=false,
  numbers=none,
  alsoletter={*?},
  morekeywords=[1]{let*,let*?,let+},
  includerangemarker=false,
  literate=
  {\ *\ }{$\,\times\:$}3
  {<-}{{{$\gets$}}}1
  {->}{{{$\tarr{}$}}}2
  {-->}{{{$/$}}}1
  {./\{}{$\{$}1
  {\}}{$\}$}1
  {_1}{{$_1$}}1
  {_2}{{$_2$}}1
  {_3}{{$_3$}}1
  {_x}{{$_x$}}1
  {.!}{}0
  {.*}{}0
  {.+}{}0
  {-:>}{$\mapsto$}1
  {--}{$\setminus$}1 
  {++}{$\cup$}1 
  {<+>}{$+$}1 
  {<->}{$-$}1
  {<.>}{$.$}1
  {<..>}{$.$}1
  {<?>}{$?$}1
  {<|=}{$\in$}1
  {!$}{}0
  {ell}{{{$\ell$}}}1
  {pi}{{$\pi$}}1
  {delta}{{{$\delta$}}}1
  {rho}{{{$\rho$}}}1
  {\\Store}{{$\delta$}}1
  {\\Perm}{$\pi$}1
  {\\VEnv}{$\gamma$}1
  {\\TimeOut}{$\TimeOut$}7
  {gamma}{{{$\gamma$}}}1
  {kappa}{{{$\kvar$}}}1
  {deltas}{{{$\overline{\delta}$}}}1
  {gammas}{{{$\overline{\gamma}$}}}1
  {kappas}{{{$\overline\kvar$}}}1
  {sigma}{{{$\sigma$}}}1
  {SCHM}{{{$\forall$}}}1
  {ty}{{$\tau$}}1
  {tybinds}{{{$\bvar{\Multi[i]\tvar}{\Multi[i]k}$}}}6
  {ks}{{$\Multi{k}$}}1
  {tys}{{$\Multi{\tau}$}}1
  {cstr}{{$C$}}1
  {<=}{$\lk$}1
  {<<=}{$\lk$}1
  {<=>}{$\equivC$}1
  {KUNR\ None}{$\kun$}1
  {RVOID}{()}2
  {RADDR\ }{}0
  {RCONST\ }{}0
  {STRELEASED}{$\StFreed$}1
  {VCreate}{Create}6
  {Imm}{$\kun$}1
  {Mut}{$\kaff$}1
  ,
}

\newcommand\lstsemrule[1]{%
  \lstinputlisting
  [style=rule,linerange=rule\ #1-(**)]
  {syntax/semanticsannotated.ml}
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> motivation-array.tex <==

\subsection{Imperative programming with linear arrays}
\label{sec:imper-progr}

The API for mutable linear arrays (shown in \cref{sig:array})
aims to safely handle manual allocation and
deallocation of arrays that may contain affine elements.
One would first use @create n v@ to create
an (unrestricted) array of size @n@ initialized with value
@v@. This value must be unrestricted as it is duplicated to
initialize all array elements. Using the @map@ function we
can transform the unrestricted elements into linear (affine)
ones. This array can be processed further using @map@ (or @set@ if
affine). The @get@ function is only applicable if the element type
is unrestricted as one element is duplicated. The @length@
function is always applicable. To @free@ an array the elements must be
affine.

To manage the different kinds of accessing the array we distinguish between constructors, destructors,
observers, and mutators.
Constructors and destructors like @create@ and @free@ manipulate the whole
array. %As with channels in \cref{sec:session-linearity},
The constructor
@create@ yields a linear resource which is consumed by @free@.
During the lifetime of the array resource @a@, we can split
off \emph{shared borrows} @&a@ that provide a read-only
view or \emph{exclusive borrows} @&!a@ for read-write views.
Observer functions such as @length@ and @get@ expect an shared borrow
argument, mutator functions such a @set@ expect
a exclusive borrow.

Each borrow is tied to a region whose lifetime is properly
contained in the lifetime of the resource.
In a region, we can split off as many shared borrows of a resource as
we like, but we can take only one exclusive borrow. In a 
subsidiary region, we can take shared borrows of any
borrow or we can take an exclusive borrow of an exclusive borrow from an
enclosing region. Borrows are confined to their regions. Inside the region,
shared borrows are unrestricted (@un@) whereas exclusive
borrows are affine (@aff@).

The code in \cref{ex:array} demonstrates a use of the API to create an
array of Fibonacci numbers as the programmer would write it. After
creation of the array, the presence of a borrow in the for loop
prevents access to the ``raw'' resource inside the loop's
body. \cref{ex:array:get} of the example contains two shared borrows
in the same expression, which forms a region by itself. These borrows
are split off the exclusive borrow used in \cref{ex:array:set}, which
belongs to the next enclosing region corresponding to the loop body.
The whole array can be returned in \cref{ex:array:return} because  the
borrows are no longer in scope. 

\begin{figure}[tp]
  \centering
  \begin{subfigure}[t]{1\linewidth}
\begin{lstlisting}
module type ARRAY = sig
  type ('a : 'k) t : lin
  val create : ('a : un) => int -> 'a -> 'a t
  val free : ('a : aff) => 'a t -> unit
  val length : &('a t) -> int
  val get : ('a : un) => &('a t) * int -> 'a
  val set : ('a : aff) => &!('a t) * int * 'a -> unit
  val map : (&'a -> 'b) -> &('a t) -> 'b t
end

module Array : ARRAY
\end{lstlisting}
    \vspace{-15pt}
    \caption{Signature}
    \label{sig:array}
  \end{subfigure}

  \begin{subfigure}[t]{1\linewidth}
\begin{lstlisting}
let mk_fib_array n =
  let a = create n 1 in
  for i = 2 to n - 1 do
    let x = get (&a, i-1) + get (&a, i-2) in(*@\label{ex:array:get}*)
    set (&!a, i, x)(*@\label{ex:array:set}*)
  done;
  a(*@\label{ex:array:return}*)
# mk_fib_array : int -> int Array.t
\end{lstlisting}
    \vspace{-10pt}
    \caption{Example of use}
    \label{ex:array}
\begin{lstlisting}[firstnumber=2]
  let a = create n 1 in
  for i = 2 to n - 1 do {|
    let x = {| get &a (i-1) + get &a (i-2) |} in(*@\label{ex:array:region:get}*)
    set &!a i x
  |} done;
\end{lstlisting}
    \vspace{-10pt}
    \caption{Excerpt of \cref{ex:array} with explicit regions}
    \label{ex:array:region}
  \end{subfigure}
  \vspace{-5pt}
  \caption{Linear arrays}
  \label{ex:array}
\end{figure}

\cref{ex:array:region} uses braces @{| ... |}@ to make the
regions of the example in \cref{ex:array} explicit.  One
region consists of the header expression of the @let@ in
\cref{ex:array:region:get}. It is contained in another region that
comprises the body of the @for@ loop. \lang guarantees that borrows
never escape the smallest enclosing region. It employs a system of
\emph{indexed kinds} like @aff_r@ and @un_r@ where
$r$ is a positive integer that corresponds to the lexical nesting
depth of regions. For instance, the type of @&!a@ in
\cref{ex:array:set} has kind @aff_1@ whereas the type of
@&a@ in \cref{ex:array:region:get} has kind
@un_2@ and the typing of the inner region is such that types with
kind indexes greater than or equal to $2$ cannot escape.
In the example, borrows cannot escape  because they are consumed
immediately by @get@ and @set@.

Region annotations are automatically inserted using
syntactic cues such as borrows and binders (see
\cref{regionannot}).  Users may manually insert regions to further restrict the range of a
borrow. In practice, region annotations are
rarely needed with common programming idioms.
% All regions for the examples in this section have been inferred.


% \begin{figure}
%   \centering
%   % \begin{subfigure}{0.6\linewidth}
% \begin{lstlisting}
% let mk_fib_array n =
%   let a = create n 1 in
%   for i = 2 to n - 1 do {|
%     let x = {| get &a (i-1) + get &a (i-2) |} in(*@\label{ex:array:region:get}*)
%     set &!a i x
%   |}
%   done;
%   a(*@\label{ex:array:return}*)
% # mk_fib_array : int -> int Array.t
% \end{lstlisting}
%     \caption{Example from \cref{ex:array} with explicit regions}
%     \label{ex:array:region}
%   % \end{subfigure}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sdtyping/sd-typing-internal-a.tex <==
\begin{mathpar}
  % \ruleSDIVar
  % \and
  % \ruleSDIVarInst
  % \and
  \ruleSDAIApp
  \and
  \ruleSDAIPair
  \and
  % \ruleSDILam
  % \and
  % \ruleSDRegion
  % \and
  % \ruleSDConst
  % \and
  % \ruleSDBorrow
  % \and
  % \ruleSDReBorrow
  % \and
  % \ruleSDILet
  % \and
  % \ruleSDIPLet
  % \and
  \ruleSDAIMatchPair
  % \and
  % \ruleSDCreate
  % \and
  % \ruleSDObserve
  % \and
  % \ruleSDUpdate
  % \and
  % \ruleSDDestroy
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> semantics.tex <==
\begin{mathpar}
  \inferrule[Lam]
  { j \fresh }
  { \ered{\closure{j}{x}{e}}{\emptyset}{\lam{x}{e}}{\closure{j}{x}{e}} }
  \and
  \inferrule[App]
  { \ered{I}{E}{f}{\closure{j}{x}{e_f}} \\
    \ered{I'}{E'}{e}{v} \\
    \ered{I''}{E''}{\subst{x}{v}{e_f}}{v_f}
  }
  { \ered{I,I',I''}{E,E',E'',\closure{j}{x}{e_f}}{\app{f}{e}}{v_f} }
  \and
  \inferrule[Let]
  { \ered{I}{E}{e}{v} \\
    \ered{I'}{E'}{\subst{x}{v}{e'}}{v'}
  }
  { \ered{I,I'}{E,E'}{\letin{x}{e}{e'}}{v'} }
\end{mathpar}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> typing.tex <==
\begin{mathpar}
  \inferrule[Var]
  { \envkind{P}{\E}{\kun} \\ \instanciate{\sigma}{\ (\qual{P}{\tau})} }
  { \hastype{P}{\E,\bvar{x}{\sigma}}{x}{\tau} }
  \and
  \inferrule[Let]
  {  \E = \esplit{\E_1}{\E_2} \\
    \hastype{Q}{\E_1}{e_1}{\tau_1} \\
    \sigma = \generalize{Q}{\E_1}{\tau_1} \\
    \hastype{P}{\E_2,\bvar{x}{\sigma}}{e_2}{\tau_2} 
  }
  { \hastype{P}{\E}{\letin{x}{e_1}{e_2}}{\tau_2} }
  \and
  \inferrule[App]
  { \E = \esplit{\E_1}{\E_2} \\
    \hastype{P}{\E_1}{e_1}{\tau'\tarr{k}\tau} \\
    \hastype{P}{\E_2}{e_2}{\tau'} }
  { \hastype{P}{\E}{\app{e_1}{e_2}}{\tau} }
  \and
  \inferrule[Lam]
  { \envkind{P}{\E}{k} \\ \hastype{P}{\E,\bvar{x}{\tau_x}}{e}{\tau} }
  { \hastype{P}{\E}{\lam{x}{e}}{\tau_x\tarr{k}{\tau}} }
  \and
  \inferrule[Fix]
  { \hastype{P}{\E}{e}{\tau\tarr{\kun}\tau} }
  { \hastype{P}{\E}{\fix{e}}{\tau} }
  \and
  \inferrule
  { \E = \E_1\cup\E_2 \\ \envkind{P}{\E_1\cap\E_2}{\kun} }
  { \E = \esplit{\E_1}{\E_2} }
\end{mathpar}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

